On Cryptographic Mechanisms for the Selective Disclosure of Verifiable Credentials

Verifiable credentials are a digital analogue of physical credentials. Their authenticity and integrity are protected by means of cryptographic techniques, and they can be presented to verifiers to reveal attributes or even predicates about the attributes included in the credential. One way to preserve privacy during presentation consists in selectively disclosing the attributes in a credential. In this paper we present the most widespread cryptographic mechanisms used to enable selective disclosure of attributes identifying two categories: the ones based on hiding commitments - e.g., mdl ISO/IEC 18013-5 - and the ones based on non-interactive zero-knowledge proofs - e.g., BBS signatures. We also include a description of the cryptographic primitives used to design such cryptographic mechanisms. We describe the design of the cryptographic mechanisms and compare them by performing an analysis on their standard maturity in terms of standardization, cryptographic agility and quantum safety, then we compare the features that they support with main focus on the unlinkability of presentations, the ability to create predicate proofs and support for threshold credential issuance. Finally we perform an experimental evaluation based on the Rust open source implementations that we have considered most relevant. In particular we evaluate the size of credentials and presentations built using different cryptographic mechanisms and the time needed to generate and verify them. We also highlight some trade-offs that must be considered in the instantiation of the cryptographic mechanisms.

==> cl_constants.tex <==
\begin{table}[!b]
	\caption{CL constants, Ursa anoncreds notation. 112-bit values taken from source code, 128-bit values from specification~\cite{anoncreds_1_spec_Ursa}.}
	\centering
	\begin{tabular}{llll}
	\toprule
	Parameter   				& Description	& \multicolumn{2}{c}{Security level}		\\
	\midrule
								&				& 112		&	128		\\
	\midrule
	\texttt{master secret}		& 				&	\multicolumn{2}{c}{256}	\\
	\texttt{e\_start}			& 				&	\multicolumn{2}{c}{596}	\\
	\texttt{e\_end\_range}			& 				&	\multicolumn{2}{c}{119}	\\
	\texttt{prime}				& RSA modulus factors	&	1024	&	1536	\\
	$v'$						& 				&	2128	&	3152	\\
	$v''$						& 				&	\multicolumn{2}{c}{2724}	\\
    \texttt{mvect}				& 				&	\multicolumn{2}{c}{592}	\\
    $\tilde{e}$					& 				&	\multicolumn{2}{c}{456}	\\
    $\tilde{v}$					& 				&	3060	&	3748	\\
    $\tilde{u}$					& 				&	\multicolumn{2}{c}{592}	\\
    $\tilde{m}$					& 				&	\multicolumn{2}{c}{593}	\\
    $\tilde{v'}$				& 				&	\multicolumn{2}{c}{673}	\\
    $\tilde{r}$					& 				&	\multicolumn{2}{c}{672}	\\
    $\tilde{\alpha}$			& 				&	\multicolumn{2}{c}{2787}	\\
    \texttt{nonce}				& 				&	\multicolumn{2}{c}{80}	\\
	\bottomrule
	\end{tabular}
	\label{tab:CL_constants}
\end{table}

\begin{comment}

\begin{table}[!b]
	\caption{CL parameter sizes.}
	\centering
	\begin{tabular}{llll}
	\toprule
	Parameter   & Description	& \multicolumn{2}{c}{Security level}		\\
	\midrule
				&				& 112		&	128		\\
	\midrule
	$l_n$    	& RSA modulus	& 2048		&	3072	\\
	$l_\Gamma$	& Commitment group modulus	&	1632	&	\\
	$l_\rho$	& Prime order subgroup of $\Gamma$	&	256	&	\\
	$l_m$		& Attributes	&	\multicolumn{2}{c}{256}	\\
	$l_{res}$	& Number reserved attributes in a certificate	&	1	&	\\
	$l_e$		& Certificate $e$ values	&	597	&	\\
    $l_e'$		& Certificate $e$ value interval	&	120	&	\\
    $l_v$		& Certificate $v$ values			&	2724	&	\\
    $l_\varnothing$	& Security parameter for statistical ZK	&	80	&	\\
    $l_k$		& Security parameter	&	160	&		\\
    $l_H$		& Fiat-Shamir hash function domain	&	256	&	256	\\
    $l_r$		& Security parameter required in credential system proof	&	80	&		\\
    $l_{pt}$	& prime number generation returns composites with probability $1-1/2^{l_{pt}}$	&	80	&	\\
    $l_{enc}$	& CS encryption security parameter, bit length of $\sqrt{n}$	&	&	\\
	\bottomrule
	\end{tabular}
	\label{tab:CL_parameters}
\end{table}

\end{comment}

==> cryptocode/sigma_protocol.tex <==
%\pseudocodeblock{
\procedureblock{Sigma protocol}{%
\\[-6pt]
%\pclb
\textbf{Prover}	\<	\<	\textbf{Verifier}	\\
%[][\hline]	\\
\<	\sendmessageright*{\TT{CMT}}	\<	\\
\<	\sendmessageleft*{\TT{CH}\sample \bin^n}	\<	\\
\<	\sendmessageright*{\TT{RSP}}	\<
}

==> image/fig_issuing.tex <==


\begin{figure}
\centering
	\includegraphics[width=.48\textwidth]{image/Issuing.pdf}
    \caption{Issuer Proof generation and verification performance test. Solid lines are median times, shaded areas are $25^{th}$ and $75^{th}$ percentile.}
	\label{fig:issuing_benchmark}
\end{figure}

==> image/fig_key_generation.tex <==
\begin{figure}
\centering
	\includegraphics[width=.48\textwidth]{image/Key_generation.pdf}

    \caption{Key generation performance test. Solid lines are median times, shaded areas are $25^{th}$ and $75^{th}$ percentile. The full CL key generation algorithm requires finding two RSA safe prime factors, which is the most expensive contribution to the performance; we highlight this by measuring CL key generation using pre-computed constant factors.}
	\label{fig:keygen_benchmark}
\end{figure}

==> image/fig_presentation_arch_benchmark.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.48\textwidth]{image/presentation_arch.pdf}
    \caption{BBS+ Presentation Proof generation and verification performance test on different CPU architectures.}
    \label{fig:presentation_arch_benchmark}
\end{figure}

==> not_used_crypto_prel.tex <==
\subsection{Commitment schemes}
In the random oracle model \cite{canetti2004random} hash functions are modeled as a random oracles, and this allows the hash functions to be the main building block of cryptographic protocols and schemes. An example of such schemes is given by \emph{commitment schemes}. Commitment schemes are meant to be the digital analogue of sealed envelops. The committer puts a message it wants to commit to inside an envelope and seals it. At this stage no one can read the message inside the envelope, but at the same time the committer can not change the content of the envelope without breaking the seal. This is one of the most used cryptographic primitives in protocol design and it is composed of two algorithms:
\begin{itemize}
\item $\TT{com:=commit(m,r)}$ the commit function takes as input a message $\TT{m}$ and a random value $\TT{r}$ and returns a commitment;

\item $\TT{verify(com, m, r)}$ the verify function returns true if its input is consistent, i.e. $\TT{com=commit(m,r)}$, false otherwise. 
\end{itemize}

We require the following security properties to hold: \emph{hiding}, which means that it should be computationally infeasible to find $\TT{m}$ given $\TT{com}$, and \emph{binding}, which means that it should be infeasible to find two pairs $\TT{(m,r), (m',r')}$ such that $\TT{m\ne m'}$ and  $\TT{commit(m,r)} = \TT{commit(m',r')}$.


\subsection{Hash functions}
\label{hash}
A \textit{hash function} is a function that satisfies the following properties: the input can be a string of any size, it produces fixed-sized outputs (called digests), it is efficiently computable. More technically, computing the hash of an $n$-bit string should require a computational effort which is $\mathcal{O}(n)$. 

We are interested in a subset of hash functions, namely \emph{cryptographically secure hash functions} \cite{dang2009nist}. These are one of the most used cryptographic primitives in protocol design due to the following additional properties:
\begin{itemize}
	\item \emph{Collision resistance}: a hash function $\HH$ is said to be collision resistant if it is infeasible to find two values $x\ne y$ for which $\HH(x)=\HH(y)$.
	\item \emph{Preimage resistance}: a hash function $\HH$ is said to be preimage resistant if, given the digest $\HH(x)$, it is infeasible to find the preimage $x$ when it is chosen at random.
	\item \emph{Second preimage resistance}: a hash function $\HH$ is said to be second preimage resistant if, given $x$, it is computationally infeasible to find $y\ne x$ such that $\HH(x)=\HH(y)$.
\end{itemize}
In this document we refer to cryptographically secure hash function by simply calling them hash function.

We now present some useful applications of hash functions that we will mention in this paper.


\subsubsection{Hash based commitment scheme}
\label{hashcom}
Let us describe a commitment scheme which exploits the properties of hash functions.

When a committer wants to commit to $\TT{m}$, it randomly generates a string $\TT{r}$ and computes the hash of the concatenation of these two values: defining $\TT{com=commit(m,r):=\HH(m || r)}$. When the committer wants to open the commitment it reveals the values $\TT{m, r}$ so that the verifier can compute $\TT{\HH(m || r)}$ and compare it with $\TT{com}$. 

This scheme satisfies the hiding property because of the preimage resistance of the underlying hash function $\HH$. In fact, if the random string $\TT{r}$ is sufficiently large, this guarantees that a computationally bounded attacker can not find the preimage of the digest $\HH(m || r)$. This scheme also satisfies the binding property because once the committer has properly created a commitment, the second preimage resistance of the underlying hash function guarantees that it can not find $\TT{m',r'}$ s.t. $\HH(\TT{m'||r'})=\HH(\TT{m||r})$ where $\TT{m'\ne m}$. Even if the committer acts maliciously from the beginning, and tries to find a value $r$ that would allow it to open the commitment verifying two distinct values $\TT{m'\ne m}$, its attack would be prevented by the collision resistance of $\HH$.

\subsubsection{Merkle trees}
\label{subsub:merkle}
A Merkle Tree is a data structure that consists of a binary tree which can be constructed taking as input an ordered set of messages that will be the \emph{leaves} of the tree and a hash function $\HH$. The second level (from the bottom) of the tree is obtained by computing the digest of each leaf (see \Cref{fig:merkle}). All the nodes in the upper levels will be constructed by computing the digest of the concatenation of two consecutive nodes of the previous level until the root is reached (i.e. the level which is composed of only one node).

This data structure is very useful for several reasons. First of all, if only the root of a Merkle tree is published, no one can trace back the underlying messages which are the leaves of the tree, thanks to the preimage resistance of the hash function adopted. Secondly, it is possible for someone who knows the underlying list of messages to prove to a verifier who has access only to the root that a given message $\TT{m}$ is included in the list. This can be done providing the verifier with the message $\TT{m}$, the only sibling of $\TT{\HH(m)}$ and for each upper level, the sibling of the node that the verifier can reconstruct using the previous information. If we consider the Merkle tree in \Cref{fig:merkle}, in order to prove to a verifier who knows only $\TT{root}$ that $a_2$ is a leaf of the tree, it must be provided with the message $a_2$, the node $b_1$ and the node $c_2$.
The verifier can compute $c_1=\HH((b_1)||\HH(a_2))$ and verify that $\HH(\HH((b_1)||\HH(a_2))||c_2)=\TT{root}$.


\begin{figure}

\centering
\begin{forest}
  [$\TT{root}:\HH(c_1||c_2)$
    [$c_1:H(b_1||b_2)$[$b_1: \HH(a_1)$[$a_1$]][$b_2:\HH(a_2)$[$a_2$]]]
    [$c_2:H(b_3||b_4)$[$b_3: \HH(a_3)$[$a_3$]][$b_4: \HH(a_4)$[$a_4$]]]
  ]
\end{forest}
\caption{Merkle tree with 4 leaves. The leaves are the nodes $a_i$. For each $i$, $d_i$ is the digest $\HH(a_i)$ di $a_i$ The root of the Merkle tree.}
\label{fig:merkle}
\end{figure}


Note that if $\TT{n}$ is the number of leaves, then the depth of the Merkle tree is $\TT{\lfloor\log_2 n\rfloor +1}$ and the dimension of the proof will be $\TT{\mathcal{O}(\log_2 n)}$ according to the output size of the underlying hash function.

In order to reduce the depth of a Merkle tree one can generalize this concept defining the $\TT{k}$-ary Merkle tree. The $\TT{k}$-ary Merkle tree has the same structure as the binary one, but the leaves and the other nodes are hashed in group of $\TT{k}$ elements to give rise to a parent and finally to the Merkle root. Note that in this case the depth of the tree is $\TT{\lfloor\log_k n\rfloor +1}$ but the proof size will be $\TT{\mathcal{O}(k\log_2 n)}$ because for each level the prover must reveal $\TT{k-1}$ digests.

\subsection{Vector commitments}
\label{prel:vectorCommitment}
\emph{Vector commitments}\atnote{This could be useful for revocation, too; let's keep it for now.} \cite{catalano2013vector} allows a user to commit to a sequence of $\TT{q}$ values rather than to a single message. 
The algorithms that define a vector commitment scheme are the following: a key generation algorithm $\TT{KeyGen(1^k,q)}$ where $\TT{k}$ is the security parameter and $\TT{q}$ is the size of the committed vector and returns a set of public parameters $\TT{pp}$; a commit algorithm $\TT{Com_{pp}(m_1,\dots,m_q)}$ that returns a commitment $\TT{C}$ and auxiliary information $\TT{aux}$; an open algorithm $\TT{Open_{pp}(m,i,aux)}$ which is run by the committer to produce a proof $\Lambda_i$ that $\TT{m}$ is the $\TT{i}$-th committed message in the vector; a verification algorithm $\TT{Ver_pp(C,m,i,\Lambda_i)}$ that accepts only if $\TT{\Lambda_i}$ is a valid proof that $\TT{C}$ is a valid commitment to $\TT{m_1,\dots,m_q}$ with $\TT{m=m_i}$. 
There is also an algorithm to update a commitment when the committer is willing to change some message in the vector committed to, and an algorithm to let any user update the proofs related to the updated messages: however, in this document we are not interested into the update functionalities.

In particular, vector commitments satisfy the following properties that can be useful in the design of verifiable credentials that implement selective disclosure:
\begin{itemize}
    \item \emph{position binding}: it is not possible to open a commitment to two different values $\TT{m_i\ne m_i'}$ at the same position $\TT{i}$;
    \item \emph{conciseness}: the size of the commitment is fixed independently on the number of elements in the vector, as well as the size of the openings;
    \item \emph{hiding}: it is infeasible to distinguish whether a vector commitment was created to a vector $\TT{(m_1,\dots,m_q)}$ or to $\TT{(m_1,\dots,m_q)}$.
\end{itemize}



Vector commitments can be also used to generate a data structure that recalls the $k$-ary Merkle tree: the \emph{Verkle tree} as we describe below.

\subsubsection{Verkle trees}
As we have mentioned in \Cref{subsub:merkle}, in a $\TT{k}$-ary Merkle trees the proof that a given value is a leaf of the tree consists on a set of $\TT{k-1}$ siblings for each level of the tree. One can reduce the depth of the tree increasing the value of $\TT{k}$, but then the proof weight increases of a factor of $\TT{k-1}$ which is the number of siblings we must reveal for each level of the tree. 




The idea behind the construction of Verkle trees is that we can construct a ($\TT{k}$-ary) Merkle tree substituting hash functions with $\TT{k}$-dimensional vector commitments. 




\subsection{Digital signatures}
\label{digSig}
\textit{Digital signatures} are cryptographic primitives supposed to be the digital analogous of a handwritten signatures on paper.

A digital signature is composed of three algorithms: $\TT{generateKeys(keySize)}$, $\TT{sign(sk,m)}$ and $\TT{verify(pk, m, sig)}$. The key generation algorithm returns a private-public key pair $\TT{(sk,pk):=generateKeys(keySize)}$. The private key is used to sign a message $\TT{m}$ and produce a signature $\TT{sig:=sign(sk,m)}$ of it. The public key is used to verify the validity of the signature of the message $\TT{m}$: $\TT{isValid:= verify(pk, m, sig)}$.
Note that the $\TT{generateKeys}$ must be a randomized algorithm because it must generate different key pairs for different users.
In contrast $\TT{verify}$ must be deterministic. 

Digital signatures must satisfy the following properties, that makes them the digital counterpart of handwritten signatures. First of all, digital signatures must not be forgiable, which means that it is infeasible for an adversary to produce the signature of a message you have not previously signed. Another property is that legitimate signatures must be always verified, hence $\TT{verify(pk,m,sign(sk,m))}=true$ for every proper key-pair $\TT{(sk,pk)=generateKeys(keySize)}$. Finally, signers cannot deny to have signed any message which verifies using their public keys: if the signature verifies, this means that the message has been signed by the owner of the associated secret key (\emph{non-repudiation property}).



==> preamble_scitepress.tex <==
\usepackage{epsfig}
\usepackage{apalike}
\usepackage{SCITEPRESS}     % Please add other packages that you may need BEFORE the SCITEPRESS.sty package.

==> preamble_sigconf.tex <==
\setcopyright{acmcopyright}
\copyrightyear{2018}
\acmYear{2018}
\acmDOI{XXXXXXX.XXXXXXX}
\acmConference[Conference acronym 'XX]{Make sure to enter the correct
  conference title from your rights confirmation emai}{June 03--05,
  2018}{Woodstock, NY}
  

==> tab_CMT_comList.tex <==
\begin{table}[!b]
\centering
\small
\caption{The hiding commitment of a VC using $\TT{\comList}$ as cryptographic mechanism.}
 \begin{tabular}{||l||} 
 \hline
 \textbf{\SDS} \\
 \hline\hline
 \textbf{List ${L}$ of commitments}:  \\
 \hspace{5pt} ${L_1=\HH(a_1||s_1)}$  \\
 \hspace{5pt} ${L_2=\HH(a_2||s_2)}$  \\
 \hspace{22pt}\vdots\\
 \hspace{5pt} ${L_m=\HH(a_m||s_m)}$ \\
 \hline
 \end{tabular}    \label{tab:comListSDS}
\end{table}

==> tab_CMT_merTree.tex <==
\begin{table}[!b]
\centering
\small
\caption{The hiding commitment of a VC using $\TT{\merTree}$ as cryptographic mechanism.}    
 \begin{tabular}{||l||} 
 \hline
 \textbf{\SDS} \\
 \hline\hline
    \textbf{Root ${R}$ of the Merkle tree}:\\
    \hspace{5pt}$R=\TT{getRoot}(a_1||s_1,a_2||s_2,\dots,a_m||s_m)$\\
    \hline
    \end{tabular}
\label{tab:merTreeSDS}
\end{table}

==> tab_efficiency.tex <==
\begin{table*}[!b]
\color{blue}
\caption{Number of operations over EC for each \SDSig: multiplication ($m$), multi-scalar multiplication ($msm$), addition ($a$), and pairing ($P$). All operations are in the group $\mathbb{G}_1$ unless otherwise subscripted with $\mathbb{G}_2$.}\label{tab:efficiency_table}\centering
    \begin{tabular}{||p{3cm}|p{3cm}|p{3cm}|p{3cm}| p{3cm}||}
        \hline
        \texttt{\textbf{Sign. Schemes}} & \texttt{Sign.}           & \texttt{Verif.}       & \texttt{PoK Gen.}       & \texttt{PoK Ver.}   \\
        \hline
        $\TT{BBS}$                    & $msm(L) + m + a$  & $msm(L) + a + a_{\mathbb{G}_2} + m_{\mathbb{G}_2} + 2P$     & $msm(L) + 3m + 2a + msm(R) + msm(2 + U)$  & $msm(R) + msm(3 + U) + 2a + 2P$    \\
        \hline
        $\TT{BBS+}  $                 & $msm(1 + L) + m + a$     & $msm(1 + L) + a + a_{\mathbb{G}_2} + m_{\mathbb{G}_2} + 2P$ & $msm(1 + L) + 3m + 2a + msm(2 + U) + msm(2)$      & $msm(R) + msm(3 + U) + msm(3) + 3a + 2P$ \\
        \hline
        $\TT{PS}$                     & $m_{\mathbb{G}_2} + rand_{\mathbb{G}_2}$ & $msm(L) + a + 2P$    & $3m_{\mathbb{G}_2} + a_{\mathbb{G}_2} + msm(1 + U)$ & $msm(2 + U) + a + msm(R) + 2P$   \\
        \hline
    \end{tabular}
\end{table*}
%m stands for scalar multiplication, i.e. given a point Q and a scalar n it is the computation nQ
%a stands for point addition, i.e. given two points Q1 and Q2 it is the computation Q1 + Q2)
%msm(n) stands for multi-scalar multiplication, i.e. a sum of n scalar multiplication.
%P stands for a pairing computation.
%rand stands for taking a random element in the group.
%L is the total number of attributes, R and U are respectively the revealed and undisclosed number of attributes.
%we assume computation over G1 if not stated otherwise.
% P > msm > m >> a >> field operations (which we do not include)
% P ~ 2msm(30), msm(30) ~ 3m, m ~ 200a, a ~ 100 field operations. Rough time esteem, expecially the first two ratios can change quite a lot, from machine and implementation. Also Operation over G2 ~ 2-3(Operation over G1).
%For Schnorr, if we need to compute a msm(n) for the commitment then we need msm(1 + n) + PA to verify.

==> tab_presentation_arch_comparison_with_4690K.tex <==
\begin{table}[!b]
\caption{Presentation Proof generation test by CPU with $n_A=33$. Times in ms are median over $n_D\leq n_A$.}
\label{tab:presentation_generation_arch_comparison} \centering
    \begin{tabular}{lrrrr}
	\toprule
	\texttt{\cm}       & 5800X     & 4690K	    & pi 4B	    & pi 3B+   \\
	\midrule
	$\TT{\merTree}-EdDSA$    & 0.0007	   & 0.0015	   & 0.0044	& 0.0143 \\
        $\TT{\merTree}-\sphincs$    & 0.0007	   & 0.0014	   & 0.0044	& 0.0174 \\
	\bbs            & 1.6508	        & 3.1944	& 11.2507	& 92.9144 \\
        PS              & 9.3314  	   & 15.6353	& 34.6971	  & 303.4390 \\
        CL             & 55.270	   & 74.7589	& 394.9524	& 1475.9164  \\
	\bottomrule
    \end{tabular}
\end{table}

\begin{table}[!b]
\caption{Presentation Proof verification test by CPU with $n_A=33$. Times in ms are median over $n_D\leq n_A$.}
\label{tab:presentation_verification_arch_comparison} \centering
    \begin{tabular}{lrrrr}
	\toprule
	\texttt{\cm}        & 5800X     & 4690K	    & pi 4B	    & pi 3B+   \\
	\midrule
	$\TT{\merTree}-EdDSA$    & 0.040	& 0.0707	& 0.2911	& 1.0715 \\
        $\TT{\merTree}-\sphincs$    & 0.4176	   & 0.6446	   & 7.0385	& 19.3736 \\
	\bbs            & 2.1360	       & 4.4014	   & 15.7105	   & 117.4054 \\
        PS               & 3.5201        & 6.1195	& 19.4249	& 210.9906 \\
        CL             & 64.969	   & 86.3935	& 456.0057	& 1687.3662  \\
	\bottomrule
    \end{tabular}
\end{table}



==> tab_speed_cm_vs_function.tex <==
\begin{table*}[!b]
\caption{Speed by mechanism for each function. Approximate orders of magnitude in ms - lower is better.}\label{tab:speed_cm_vs_function} \centering
    \begin{tabular}{lrrrrr}
	\toprule
	Mechanism          & \keyGen     & \genIssProof	    & \verIssProof	    & \genHolderProof   & \verPresProof  \\
	\midrule
    $\TT{\merTree}$    & -2	& -1	& -1	& -3     & -1    \\
    CL & 4	& 2	& 2	& 2     & 2    \\
    BBS+  & 0	& 0	& 1	& 1     & 1     \\
	\bottomrule
    \end{tabular}
\end{table*}



==> tab_speed_cm_vs_function_transpose.tex <==
\begin{table}[!b]
\caption{Speed by mechanism for each function. Approximate orders of magnitude in ms - lower is faster.}
\label{tab:speed_cm_vs_function} \centering
    \begin{tabular}{lrrr}
	\toprule
	Function          &   $\TT{\merTree}$   & CL	    & BBS+	    \\
	\midrule
    \texttt{\keyGen}         & -2	& 4    & 0    \\
    \texttt{\genIssProof}    & -1	& 2    & 0    \\
    \texttt{\verIssProof}    & -1	& 2    & 1    \\
    \texttt{\genHolderProof} & -3	& 2    & 1    \\
    \texttt{\verPresProof}  & -1	& 2    & 1    \\
	\bottomrule
    \end{tabular}
\end{table}



==> tab_summary_analysis.tex <==

\begin{table}[!b]

\caption{\texttt{\cm} assessment summary. }\label{tab:summary_analysis} \centering
    \begin{tabular}{lcccc}
	\toprule
	Feature          & \texttt{\comList}    &   \texttt{\merTree}   & \texttt{\CL}	    & \texttt{\BBS}	    \\
	\midrule
    Standard        &  \high    & \meh     & \low    & \meh    \\
    Agile         &  \high    & \high     & \lowww    & \high    \\
    Unlinkable   &  \meh    & \meh     & \high    & \high    \\
    Predicates      &  \meh    & \meh 	& \high    & \high    \\
    Fast           &  \highhh    & \highhh 	& \loww   & \low    \\
    Compact         &  \low    & \high     & \loww    & \high    \\
	\bottomrule
    \end{tabular}
\end{table}



==> tab_summary_analysis_textcolor.tex <==

\begin{table}[!b]

\caption{\texttt{\cm} assessment summary. }\label{tab:summary_analysis} \centering
    \begin{tabular}{lcccc}
	\toprule
	Feature          & \texttt{\comList}    &   \texttt{\merTree}   & \texttt{\CL}	    & \texttt{\BBS}	    \\
	\midrule
    Standard        &  \chigh    & \cmeh     & \clow    & \cmeh    \\
    Agile         &  \chigh    & \chigh     & \clowww    & \chigh    \\
    Unlinkable   &  \cmeh    & \cmeh     & \chigh    & \chigh    \\
    Predicates      &  \cmeh    & \cmeh 	& \chigh    & \chigh    \\
    Fast           &  \chighhh    & \chighhh 	& \cloww   & \clow    \\
    Compact         &  \clow    & \chigh     & \cloww    & \chigh    \\
	\bottomrule
    \end{tabular}
\end{table}


==> tab_summary_analysis_words.tex <==

\begin{table}[!b]
\small
\caption{\texttt{\cm} assessment summary. }\label{tab:summary_analysis} \centering
    \begin{tabular}{lllll}
	\toprule
	Feature          & \texttt{\comList}    &   \texttt{\merTree}   & \texttt{\CL}	    & \texttt{\BBS}	    \\
	\midrule
    Standard        &  Yes    & Draft     & No    & Draft    \\
    Agility         &  Yes    & Yes     & No    & Yes    \\
    Unlinkable   &  Iss.    & Iss.     & Pres.    & Pres.    \\
    Predicates      &  Iss.    & Iss. 	& Pres.    & Pres.    \\
    Speed           &  High    & High 	& Low   & Med.    \\
    Compact         &  Med.    & High     & Low    & High    \\
	\bottomrule
    \end{tabular}
\end{table}


==> tab_summary_analysis_wordscolor.tex <==

\begin{table}[!b]
\small
\caption{\texttt{\cm} assessment summary. }\label{tab:summary_analysis} \centering
    \begin{tabular}{lllll}
	\toprule
	Feature          & \texttt{\comList}    &   \texttt{\merTree}   & \texttt{\CL}	    & \texttt{\BBS}	    \\
	\midrule
    Standard        &  \aquamarine{Yes}    & \dandelion{Draft}     & \caramel{No}    & \dandelion{Draft}    \\
    Agility         &  \aquamarine{Yes}    & \aquamarine{Yes}     & \caramel{No}    & \aquamarine{Yes}    \\
    Unlinkable   &  \dandelion{Iss.}    & \dandelion{Iss.}     & \aquamarine{Pres.}    & \aquamarine{Pres.}    \\
    Predicates      &  \dandelion{Iss.}    & \dandelion{Iss.} 	& \aquamarine{Pres.}    & \aquamarine{Pres.}    \\
    Speed           &  \aquamarine{High}    & \aquamarine{High} 	& \caramel{Low}   & \dandelion{Med.}    \\
    Compact         &  \dandelion{Med.}    & \aquamarine{High}     & \caramel{Low}    & \aquamarine{High}    \\
	\bottomrule
    \end{tabular}
\end{table}


==> zero-knowledge_proofs.tex <==
A Zero-Knowledge proof (ZKP) is a cryptographic protocol that allows a prover to convince a verifier of the truth of a statement, without revealing anything else to the verifier.

In order to prove that a protocol is indeed a zero knowledge proof of knowledge of a secret we must prove that the following three properties that we state informally hold:
\begin{itemize}
    \item \emph{Completeness}: which implies that if the prover executes the protocol instructions then an honest verifier would accept its proof.
    \item \emph{Soundness}: which implies that an attacker who does not know the secret, with overwhelming probability will not be able to convince any verifier that it knows the secret.
    \item \emph{Zero-Knowledge}: which implies that from an interaction it is not possible to learn anything about the secret.
\end{itemize}
Proving the completeness property in most cases is straightforward. 

A standard way to prove the soundness property consists into creating a \emph{knowledge extractor} which is an algorithm that, interacting with the attacker, is capable to extract the secret from accepted interactions. This is possible since the knowledge extractor has direct access to the execution environment of the attacker and in particular it can \emph{rewind} the attacker state. In the real world, since one cannot rewind an honest prover, an attacker cannot use this strategy to extract the secret from the prover.
However, if such a knowledge extractor exists, then it means that the prover actually knows the secret.

Finally, in order to prove that a protocol satisfies the zero-knowledge property, it is necessary to create another algorithm called \emph{simulator} which does not know the secret. The simulator must be able to generate valid transcripts of conversation between prover and verifier. The messages can be created in any possible way, the only thing that matters is that the transcripts created by the simulator result to be valid, i.e. the transcript, given in input to the verification algorithm of the verifier, results to be accepted. If such a simulator exists, then no one can learn anything about the secret by just observing an interaction between a prover and a verifier, not even the verifier. In fact a valid transcript can be produced even without knowledge of the secret. 

To summarize, if the properties above hold, when a verifier interacts with a prover, the verifier will not be able to extract any information from the interaction since there exists a simulator capable to create valid transcript. However, since the verifier knows that the transcript is being created having the prover answering its randomly generated challenge, then thanks to the existence of a knowledge extractor, the verifier can be assured that the prover knows the actual secret. 

An early example of ZKP is Schnorr identification scheme that allows a prover to prove a verifier the knowledge of a discrete logarithm $\TT{y=g^x}$ for some $\TT{x\in\mathbb{Z}_p}$ and $\TT{\mathbb{G}=<g>}$ of prime order $\TT{p}$. We have presented this protocol as an identification scheme that we have claimed to be secure is a zero-knowledge proof of a discrete logarithm and the simulator works as follows: randomly pick an element in $\mathbb{G}$ and let it be the 






